A Novel Design for Advanced 5G Deployment Environments with Virtualized Resources at Vehicular and MEC Nodes

IoT and edge computing are profoundly changing the information era, bringing a hyper-connected and context-aware computing environment to reality. Connected vehicles are a critical outcome of this synergy, allowing for the seamless interconnection of autonomous mobile/fixed objects, giving rise to a decentralized vehicle-to-everything (V2X) paradigm. On this front, the European Telecommunications Standards Institute (ETSI) proposed the Multi-Access Edge Computing (MEC) standard, addressing the execution of cloud-like services at the very edge of the infrastructure, thus facilitating the support of low-latency services at the far-edge. In this article, we go a step further and propose a novel ETSI MEC-compliant architecture that fully exploits the synergies between the edge and far-edge, extending the pool of virtualized resources available at MEC nodes with vehicular ones found in the vicinity. In particular, our approach allows vehicle entities to access and partake in a negotiation process embodying a rewarding scheme, while addressing resource volatility as vehicles join and leave the resource pool. To demonstrate the viability and flexibility of our proposed approach, we have built an ETSI MEC-compliant simulation model, which could be tailored to distribute application requests based on the availability of both local and remote resources, managing their transparent migration and execution. In addition, the paper reports on the experimental validation of our proposal in a 5G network setting, contrasting different service delivery modes, by highlighting the potential of the dynamic exploitation of far-edge vehicular resources.

==> analysis.tex <==
\section{Real-world Data Analysis}
Fig.~\ref{fig:arch} shows the deployment of our framework in a vehicular cloud context, where cars provide their onboard resources and UEs request \mec{} service execution. As mentioned in section \af{Add reference to design section}, the \mechost{} subscribes to an AoI (e.g., parking lot) to be aware of available resources in that area.  In this context, parked cars may leave the parking lot once their resources have been allocated, thus generating service interruption.To deal with this problem, the MEC-H starts the migration procedure by transferring all the information needed in the new location to restore the execution. However, in the case of stateful \mec~apps, migrations generate a downtime period in which the app involved becomes unavailable. Hence, to measure this metric we created a scenario where vehicles enter and leave a parking lot, and UEs request edge applications during day hours. To make this scenario as close as possible to reality, we based our study on two real-world datasets. The dataset in~\cite{arnhemdataset} provides car transactions of three parking garages in the city of Arnhem. It reports information about cars entering and leaving times of each parking lot. On the other hand, the dataset in~\cite{bolognadataset} describes the usage of public WiFi networks in the city of Bologna. It records the number of users joining the WiFi network each day. We analyzed each parking garage and each network available to find a relationship between these datasets. Thus, we selected one parking garage context and location and filtered Bologna's dataset using this information. The location chosen is the \textit{Ceentral garage}, a parking area close to the train station of Arnhem. Therefore, we extracted data related to WiFi network usage within the train station of Bologna. Once we gathered these data, we studied the distributions of the occupancy time, i.e., the time a car remains parked, the average number of cars entering per hour, and the average number of UEs joining the network per hour. Based on the fitted distribution found for the occupancy time, we decided to approximate it with a normal distribution with mean $\mu=202.80$ minutes and standard deviation $\sigma=135.07$. Other metrics, i.e., the number of cars and UEs joining the area per hour, are described by Poisson distributions as these events are independent of each other and occur randomly within a hour but with a known mean rate.

We used the distributions obtained to feed an event-based simulator that generates cars and UEs in a 5G network. The deployment of this scenario allows us to analyze the trend of migrations needed during the day, to evaluate the performance of our framework during migration caused by cars leaving a parking lot. \af{We give evaluation details in the next section}
% In this environment, each UE generates a \mec{} compliant request for \mec{} app execution. Thus, 

% \af{Cite this \cite{6143927}}

==> drafts.tex <==
\subsection{OMNET ++}
\omnetpp{}\cite{omnetwebsite} is a discrete event simulator framework based on message exchange and used primarily to model and build simulations for generic purposes. However, its highly modular architecture has allowed it to gain popularity within the scientific community as a network simulation tool and, to date, it is supported by several third-party projects that continues to extend it with new models.
The modularity of \omnetpp{} comes from the presence of a programming system based on components called modules that, if properly designed, can be reused in an easy and effective way. The basic modules are known as simple modules; they represent the active elements underlying a simulation and, with each one, there is an associated user-written C++ script that defines its behavior. Simple modules can be assembled to create new modules, called compounds, up to form a hierarchical structure that represents the final model or network of the simulation. Unlike the former, compound modules are defined only in terms of structure through a proprietary declarative language called Network Description (\ned{}) that describes the submodules, parameters, and interconnections. Each module can communicate with others through the exchange of messages that can contain arbitrarily complex data structures. Messages always have their origin and destination in a simple module, where processing takes place, and travel within the hierarchical structure through entry points called gates. Gates can represent either an entry point (input gate) or an exit point (output gate) for a module's messages and are connected respecting the network hierarchy, whereby a module's gates can only be connected to modules at the same level of the hierarchy or to its direct children. The discrete event simulator feature derives from the fact that the state of the simulation changes only as events occur, which in this case corresponds to the arrival of messages. It follows that the simulation time advances only at the reception of a message, and therefore \omnetpp{}+ neglects any processing time, i.e., the time to execute the code of the simple modules, allowing it to collect metrics and rely solely on the communication time between modules.
Finally, the \omnetpp{} framework also exploits events to implement a statistics logging system, which is useful for defining custom metrics that can be collected during the execution of a simulation, making the job of results assessment easier.

\subsection{Simu5G}
Simu5G \cite{simu5g_1} is a simulation library for the \omnetpp{} framework containing a collection of models and components useful for creating arbitrarily complex end-to-end scenarios involving 5G technology. Simu5G models both the core network and the RAN of a 5G network through the implementation of 3GPP-compliant protocols and a physical transmission system based on a set of customizable channels. The simulations created with this library can also leverage heterogeneous models related to gNBs antennas that use the X2 interface to support handover and inter-cell interference coordination. However, Simu5G can be used to analyze transition scenarios from 4G to 5G networks due to the ability to use dual connectivity between eNB and gNB antennas. Among the various implemented models Simu5G provides an implementation of the ETSI MEC standard with its main components (MEC Orchestrator, MEC host, etc.) and the ability to create applications that communicate via ETSI-compliant interfaces with other elements of the MEC ecosystem. Running applications can either be self-contained or take advantage of the presence of standard MEC services; currently, the framework implements the Location Service and the Radio Network Interface Service. A significant feature of the tool is that Simu5G can also be employed as a real-time emulator. It makes possible to arbitrarily replace simulation elements (5G network, MEC elements, etc.) with real devices and thus use the same code for simulation and prototyping. In addition, the use of physical components also allows for more realistic and reliable data collection.
